Rotor Thermal Monitoring Scheme for Direct-Torque-Controlled Interior Permanent Magnet Synchronous Machines via High-Frequency Rotating Flux or Torque Injection

Interior permanent magnet synchronous machine drives are widely employed in electric traction systems and various industrial processes. However, prolonged exposure to high temperatures while operating can demagnetize the permanent magnets to the point of irreversible demagnetization. In addition, direct measurements with infrared sensors or contact-type sensors with wireless communication can be expensive and intrusive to the motor drive systems. This paper thus proposes a nonintrusive thermal monitoring scheme for the permanent magnets inside the direct-torque-controlled interior permanent magnet synchronous machines. By applying an external high-frequency rotating flux or torque signal to the hysteresis torque controller in the motor drive, the high-frequency currents can be injected into the stator windings. The permanent magnet temperature can thus be monitored based on the induced high-frequency resistance. The nonintrusive nature of the method is indicated by the elimination of the extra sensors and no hardware change to the existing system. Finally, the effectiveness of the proposed method is validated with experimental results.

==> biography.tex <==
\vskip 0pt plus -1fil
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Shen.pdf}}]{Shen Zhang}
(S'13) received the B.S. degree with the highest honor in electrical engineering from Harbin Institute of Technology, Harbin, China, in 2014. He is currently working toward the Ph.D. degree at the School of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta, GA. 

Since August 2014, he has been working on the design, optimization and condition monitoring of electric machines in the electric power group of the Georgia Institute of Technology. He was a research intern at Eaton China Innovation Center, Shanghai, China, in 2014, where he received the Best Intern Award. In 2016 summer, he was a research intern at Tesla Motors, Inc., Fremont, CA. In 2018 summer, he was a research intern at Mitsubishi Electric Research Laboratories (MERL), Cambridge, MA. His research interests include design, control, condition monitoring and diagnostics of electric machines, control of power electronics, powertrain engineering in electric vehicles,  machine learning and data mining applied to energy systems.
\end{IEEEbiography}
%
\vskip 0pt plus -1fil
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Sufei.pdf}}]{Sufei Li}
(S'15) received the B.S. degree in electrical engineering from Shanghai Jiao Tong University, Shanghai, China, in 2011, and the dual M.S. degree in electrical and computer engineering from Shanghai Jiao Tong University and Georgia Institute of Technology, Atlanta, GA, USA, in 2014. He is currently pursuing the Ph.D. degree at the School of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta.

Since August 2014, he has been working on the design and control of electric machines as a graduate Research or Teaching Assistant in the electric power group at Georgia Institute of Technology. In summer 2016, he was a Graduate Summer Intern with Siemens Energy Inc., Charlotte, NC. His research interests include the multi-physics modeling, design, control and condition monitoring of electric machines, computational intelligence applied to electric machines and power systems, and the control of power converters. He served as the President of the Georgia Institute of Technology Student Branch Chapter of the IEEE Power \& Energy Society from 2015 to 2016.
\end{IEEEbiography}
%
\vskip 0pt plus -1fil
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Lijun.pdf}}]{Lijun He}
Lijun He (S'12--M'16) received the B.S. degree in electrical engineering from Tsinghua University, Beijing, China, in 2011. and the M.S. and Ph.D. degrees in electrical engineering from the Georgia Institute of Technology, Atlanta, GA, USA, in 2013 and 2015, respectively. 

Since 2016, she has been with the GE Global Research Center, Niskayuna, NY, USA, as a Lead Electrical Engineer. Her research interests include control, design and condition monitoring of electric machines, multiphysics modeling work of protection devices in distributed power system, and renewable energy.
\end{IEEEbiography}
%
\vskip 0pt plus -1fil

% Prof. Restrepo
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Restrepo.pdf}}]{Jose A. Restrepo}
(S'89-M'92-SM'18) received the B.Sc. and M.Sc. degrees in electronics engineering from Universidad Simon Bolivar, Caracas, Venezuela, in 1988 and 1991, respectively, and the Ph.D. degree from the University of Manchester Institute of Science and Technology, Manchester, U.K., in 1996.

He was a Visiting Professor with the School of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta, GA, USA, in 2002 and 2010, respectively. He is currently a retired Professor of electronics engineering with the Departamento de Electronica y Circuitos, Universidad Simon Bolivar, Caracas, and also a Research Professor with the Faculty of Engineering and Applied Sciences, Universidad Tecnica del Norte, Ibarra, Ecuador. His research interests include power electronics, advanced control of electrical machines, artificial intelligence, power quality, and digital signal processors applied to motion control.

\end{IEEEbiography}

% % Dr./ Harley
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Harley.pdf}}]{Ronald G. Harley}
% (M'77--SM'86--F'92--LF'09) received the M.Sc.Eng. degree (cum laude) in electrical engineering from the University of Pretoria, Pretoria, South Africa, in 1965, and the Ph.D. degree in electrical engineering from London University, London, U.K., in 1969. 

% In 1971, he was appointed to the Chair of Electrical Machines and Power Systems at the University of Natal, Durban, South Africa. He is currently the Duke Power Company Distinguished Professor and Regents Professor with the School of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta. He has coauthored some 600 papers in refereed journals and international conferences and is the holder of nine patents. His research interests include the dynamic behavior and condition monitoring of electric machines, motor drives, power systems and their components, and controlling them by the use of power electronics and intelligent control algorithms.

% Dr. Harley is a Fellow of the Institution of Electrical Engineers, U.K. He is also a Fellow of the Royal Society in South Africa and a Founder Member of the Academy of Science in South Africa formed in 1994. He was the recipient of the Cyrill Veinott Award in 2005 from the IEEE Power Engineering Society for “Outstanding contributions to the field of electromechanical energy conversion”. In 2009, he received the IEEE Richard H. Kaufmann field award with citation “For contributions to monitoring, control and optimization of electrical processes including electrical machines and power networks.”

% \end{IEEEbiography}
%
\vskip 0pt plus -1fil
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Habetler.pdf}}]{Thomas G. Habetler}
(S'82--M'83--SM'92--F'02) received the B.S.E.E. degree in 1981 and the M.S. degree in 1984, both in electrical engineering, from Marquette University, Milwaukee, WI, and the Ph.D. degree from the University of Wisconsin-Madison, in 1989.

From 1983 to 1985 he was employed by the Electro-Motive Division of General Motors as a Project Engineer. Since 1989, he was with the Georgia Institute of Technology, Atlanta, where he is currently a Professor of Electrical and Computer Engineering. His research interests are in electric machine protection and condition monitoring, switching converter technology, and drives. He has published over 300 technical papers in the field. He is a regular consultant to industry in the field of condition-based diagnostics for electrical systems.

Dr. Habetler was the inaugural recipient of the IEEE-PELS “Diagnostics Achievement Award,” and a recipient of the EPE-PEMC “Outstanding Achievement Award.” the 2012 IEEE Power Electronics Society Harry A. Owen Distinguished Service Award, the 2012 IEEE Industry Application Society Gerald Kliman Innovator Award. He has also received one Transactions and four conference prize paper awards from the Industry Applications Society. He has served on the IEEE Board of Directors as the Division II Director, and on the Technical Activities Board, the Member and Geographic Activities Board, as a Director of IEEE-USA, and is a past president of the Power Electronics Society. He has also served as an Associate Editor for the \textsc{IEEE Transactions on Power Electronics}.

\end{IEEEbiography}
